Pseudo Labelling for Enhanced Masked Autoencoders

Masked Image Modeling (MIM)-based models, such as SdAE, CAE, GreenMIM, and MixAE, have explored different strategies to enhance the performance of Masked Autoencoders (MAE) by modifying prediction, loss functions, or incorporating additional architectural components. In this paper, we propose an enhanced approach that boosts MAE performance by integrating pseudo labelling for both class and data tokens, alongside replacing the traditional pixel-level reconstruction with token-level reconstruction. This strategy uses cluster assignments as pseudo labels to promote instance-level discrimination within the network, while token reconstruction requires generation of discrete tokens encapturing local context. The targets for pseudo labelling and reconstruction needs to be generated by a teacher network. To disentangle the generation of target pseudo labels and the reconstruction of the token features, we decouple the teacher into two distinct models, where one serves as a labelling teacher and the other as a reconstruction teacher. This separation proves empirically superior to a single teacher, while having negligible impact on throughput and memory consumption. Incorporating pseudo-labelling as an auxiliary task has demonstrated notable improvements in ImageNet-1K and other downstream tasks, including classification, semantic segmentation, and detection.

==> back <==
\begin{table*}[h]
\centering
\begin{tabular}{l | c c c c c c c}
 Method & Backbone & FLOPs (G) & Param. (M) & Supervision & Pretrain Epochs & Finetuning & Linear Evaluation\\
 \hline
 ViT\cite{vit} & ViT-B & 17.5 & 86 & RGB & - & 79.9 & -\\  
 BEiT\cite{beit} & ViT-B & 17.6 & 87 & DALL-E & 800 & 83.2 & 37.6\\
 CAE\cite{cae} & ViT-B & 17.5 & 86 & DALL-E & 800 & 83.6 & 68.6\\
 MaskFeat\cite{maskfeat} & ViT-B & 17.5 & 86 & HOG & 300 & 83.6 & -\\
 iBOT\cite{ibot} & ViT-B & 17.5 & 86 & Momentum & 1600 & 84.0 & -\\
 MCSSL\cite{mcssl} & ViT-B & 17.5 & 86 & Momentum & 800 & 84.0 & -\\
 MAE\cite{mae} & ViT-B & 17.5 & 86 & Momentum & 800 & 83.6 & 67.8\\
 SdAE\cite{sdae} & ViT-B & 17.5 & 86 & Momentum & 300 & 84.1 & 64.9\\
 Ours & ViT-B & 17.5 & 86 & Momentum & 300 & 84.1 & -\\
\end{tabular}
\caption{Temporary Table for results on Imagenet-1K.}
\end{table*}



\begin{figure*}
      \centering
      \begin{subfigure}[b]{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/i.png}
		\caption{Input image}
		\label{fig:i}
	   \end{subfigure}
	   \begin{subfigure}{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/n3.png}
		\caption{Layer3(w/o hier.)}
		\label{fig:o3}
	   \end{subfigure}
	   \begin{subfigure}{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/n5.png}
		\caption{Layer5(w/o hier.)}
		\label{fig:o3}
	    \end{subfigure}
     \begin{subfigure}{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/n7.png}
		\caption{Layer7(w/o hier.)}
		\label{fig:o3}
	    \end{subfigure}
     \begin{subfigure}{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/n11.png}
		\caption{Layer11(w/o hier.)}
		\label{fig:o3}
	    \end{subfigure}
	\vfill
      \begin{subfigure}[b]{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/i.png}
		\caption{Input image}
		\label{fig:i1}
	   \end{subfigure}
	     \begin{subfigure}{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/i3.png}
		\caption{Layer3((with hier.)}
		\label{fig:o3}
	   \end{subfigure}
	   \begin{subfigure}{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/i5.png}
		\caption{Layer5(with hier.)}
		\label{fig:o3}
	    \end{subfigure}
     \begin{subfigure}{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/i7.png}
		\caption{Layer7(with hier.)}
		\label{fig:o3}
	    \end{subfigure}
     \begin{subfigure}{0.15\linewidth}
		\includegraphics[width=\linewidth]{figs/i11.png}
		\caption{Layer11(with hier.)}
		\label{fig:o3}
	    \end{subfigure}
	\caption{Visualisation of attention matrix on Imagenet-1K validation set for several layers for our method with and without hierarchical connections. Using hierarchical connections produce a lower attention spread across all layers except the last layer which shows the capability of the network to attend to finer local details.}
	\label{fig:attn}
\end{figure*}


\begin{figure*}
      \centering
      \begin{subfigure}[b]{0.2\linewidth}
		\includegraphics[width=\linewidth]{figs/p1.png}
		\caption{Input image}
		\label{fig:i}
	   \end{subfigure}
	  \begin{subfigure}{0.2\linewidth}
		\includegraphics[width=\linewidth]{figs/pa1.png}
		\caption{(with hier.)}
		\label{fig:o3}
	   \end{subfigure}
        \begin{subfigure}{0.2\linewidth}
		\includegraphics[width=\linewidth]{figs/pb1.png}
		\caption{(w/o hier.)}
		\label{fig:o3}
	  \end{subfigure}
	\vfill
      \begin{subfigure}[b]{0.2\linewidth}
		\includegraphics[width=\linewidth]{figs/p2.png}
		\caption{Input image}
		\label{fig:i}
	   \end{subfigure}
	  \begin{subfigure}{0.2\linewidth}
		\includegraphics[width=\linewidth]{figs/pa2.png}
		\caption{(with hier.)}
		\label{fig:o3}
	   \end{subfigure}
        \begin{subfigure}{0.2\linewidth}
		\includegraphics[width=\linewidth]{figs/pb2.png}
		\caption{(w/o hier.)}
		\label{fig:o3}
	  \end{subfigure}
	\caption{Visualisation of attention of a patch located at centre position marked with light green circle. The leftmost column represents input images, middle column represent our model with hierarchical connections (default) and the last column represents our model without hierarchical connections.}
	\label{fig:attn}
\end{figure*}

==> sec/0_abstract.tex <==
\begin{abstract}
Masked Image Modeling(MIM) based models like SdAE, CAE, GreenMIM, MixAE have explored different ways to improve the performance of MAE by modifying prediction, loss or introducing additional architectural components. We explore an alternative procedure that enhances MAE by introducing pseudo labelling as an auxiliary pretext task in addition to replacing pixel level reconstruction with reconstruction at token level. The pseudo labelling task involves generating cluster assignments which act as pseudo labels where as token reconstruction requires generation of discrete tokens. The targets for pseudo labelling and reconstruction needs to be generated by a teacher network. To disentangle the target cluster assignments and token representations generation we decouple the teacher into two distinct models where one acts as a reconstruction teacher and the other as a clustering teacher. This disentanglement is superior to a single teacher which is proved empirically with experiments. The addition of auxiliary task is done at both class and patch level which imbues the network with instance level discrimination.  Clustering as an auxiliary task brings improvements in Imagenet1-K along with other downstream tasks like classification, semantic segmentation, detection. In addition we also show improvement in Linear evaluation from other MIM based method with the simple addition of the auxiliary pretext task.


%However naive combination of token level reconstruction and cluster pretext task does not directly improve performance on downstream tasks. We disentangle token 

%The teacher used for reconstruction requires stable targets and needs less frequent EMA updates whereas the teacher used for clustering benefits from more frequent updates. Our model introduces a novel dual teacher encoder to generate cluster assignments and target tokens separately. The student is trained with a combined token level reconstruction loss and clustering loss at patch and class level.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Masked Language modeling(MLM) introduced in Bert\cite{bert} has shown that masking and predicting the masked tokens provides for a good pretext task for language. GMML\cite{gmml} introduced in SiT\cite{sit} has proved that masking large regions of image with noise, alien concepts and reconstructing the masked regions provides for a better pretext task that works very well in low data regime. MAE\cite{mae}, SimMIM\cite{simmim}, BEiT\cite{beit} continued the idea of masked image modelling(MIM) either at pixel level or token level to generate state of the art models which works across different downstream tasks.

%Different from MIM based methods instance discrimination methods\cite{dino, mcssl, sit, simclr, simclr2, moco, mocov2, mocov3} explore either clustering or contrastive learning as a pretext task for self supervised learning(SSL). 
Masked Auto Encoders\cite{mae} employ a sparse encoder where the masked regions are dropped and corresponding mask tokens are added only in decoder layers to reconstruct the original image. The sparsity makes MAE more efficient pretraining strategy and thus has been explored by different works\cite{sdae, cae, evolvedmae} to improve it further. SdAE\cite{sdae} replaces pixel level reconstruction of MAE with token level. \cite{evolvedmae} propose to adopt masking based on attention to further produce good representations with MAE. CAE\cite{cae} adopts an auxiliary task of mask representation prediction which is similar to token level prediction in addition to reconstruction at pixel level utilised by MAE. Addition of auxiliary task which introduces instance level discrimination to MAE has not been explored.

\begin{figure*}[h]
\centering
\includegraphics[width=0.9\linewidth]{figs/arch.pdf}
\caption{Overview of proposed architecture. The model consists of two disentangled teacher encoders and a student encoder with a decoder attached. The student encoder is sparse and process only the unmasked regions of the input. Both reconstruction teacher and cluster teacher process multi fold input which is generated by splitting the masked regions of the input. Cluster teacher generates cluster assignments and reconstruction teacher generates target tokens for all the folds. Our multi fold clustering is done on the patch and class tokens but the depiction of class token is skipped for simplicity. Finally the total loss is the sum of cross entropy loss between teacher, student cluster assignments and cosine similarity loss between the student prediction, teacher target token representations.}
\label{fig:arch_overview}
\end{figure*}

In contrast addition of MIM to instance level discrimination methods has been explored by previous works\cite{sit, mcssl}. SiT\cite{sit} explored the addition of pixel level reconstruction to SimCLR\cite{simclr} and improved the performance further. MCSSL\cite{mcssl} explored pixel level reconstruction with GMML\cite{gmml} and extended DINO\cite{dino} to patches. The above methods do not have sparse encoders like MAE and utilise large amount of mask tokens or noise (around $50\%$) for masking which do not occur during finetuning. MAE\cite{mae} does not suffer from this discrepancy as it drops significant portion of the input($75\%$) rather than replacing with mask tokens which in turn also makes it efficient. 

In this work, we develop an approach to Mask Image Modelling(MIM) which is sparse in the encoder similar to MAE but does reconstruction in token embedding space rather than pixel space. The targets for the reconstruction task are generated by a reconstruction teacher. Additionally to add discriminative information to our newly designed model we add an auxiliary pseudo labelling pretext task. The pseudo labels are generated using clustering from a cluster teacher. Noticably, we differ from other multi pretext task models like \cite{sit, mcssl} and other clustering methods \cite{ibot, dino, swav, msn} with the use of two teachers for each pretext task which disentangles the outputs generated from both the pretext tasks. SdAE\cite{sdae} introduces multi fold masking while passing inputs to the teacher to maintain similar mutual information between teacher and student. We propose a multi fold clustering strategy and extend it to class and patch tokens which shows an noticeable improvement in the downstream tasks. Additionally we explore improving the ViT\cite{vit} encoder in both the student and teachers by considering inputs from multiple levels of feature hierarchy to generate encoder outputs. This enables us to capture finegrained information present in lower levels and semantic information present in the higher levels of the encoder. Figure(\ref{fig:arch_overview}) provides an overview of our entire architecture.

The following sections are organised as follows: Section \ref{sec:related_work} provides a brief overview of various self supervised models particulary relating to masked image modelling(MIM). In Section \ref{sec:methodology}, we elaborate on our proposed methodology and provide details of individual components. Section \ref{sec:experiments} provides the experimental settings and the results on classification, segmentation and detection. Finally, Section \ref{sec:conclusion} concludes the paper by providing the conclusion and possible future directions.





==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related_work}
Recent methods for SSL are based on either masked image modelling(MIM) or clustering or contrastive methods. Cluster/Contrastive methods focus on global semantic representation and can be broadly classified as instance discrimination methods. BERT\cite{bert} introduced the concept of masking random tokens in a transformer input and predicting those masked tokens. Masked Image Modelling(MIM) has been introduced in GMML\cite{gmml} proposed in SiT\cite{sit}. It considers random blocks of an image for masks and predicts the representation in pixel space. MAE\cite{mae} explored the concept of sparse encoder where the masked tokens are dropped and reconstruction is done with the help of a transformer based decoder. The reconstruction is done at pixel level which are normalised. SimMIM explores MIM in pixel space with a light weight decoder and an encoder which does not drop masked tokens. BeiT\cite{beit} explored masked image modelling through reconstruction at token level. The codebook for the target token representation is generated by a dVAE which has to be trained separately. MAE is compute efficient compared to other methods like \cite{simmim, beit} because of sparse processing of only visible tokens in encoder. 

Several methods \cite{sdae, cae, evolvedmae, mixmae, greenmim, ummae} have proposed enhancements to MAE by adding different components or applying it to various hierarchical architectures. UM-MAE\cite{ummae} proposes a two stage masking strategy for making MAE pretraining viable for hierarchical architectures like PVT\cite{pvt}, Swin\cite{swin}. GreenMIM\cite{greenmim} applies MAE on hierarchical models with the help of a new window attention mechanism and dynamic programming. MixMAE\cite{mixmae} proposes an simple strategy for applying MAE to hierarchical models by considering mixing of several images as masking. CAE\cite{cae} separates the pretraining tasks from learning representations with the help of an additional alignment module. \cite{evolvedmae} proposes a masking strategy based on the attention maps of the encoder to capture better semantics. This new masking strategy learns objects parts effectively further enhancing MAE. 

Addition of MIM as an auxiliary task to enhance the SSL models has been studied in case of instance discrimination models\cite{sit, gmml}. SiT\cite{sit} considers addition of GMML\cite{gmml} which reconstructs the image in original pixel space as auxiliary task to SimCLR\cite{simclr} to enhance the representations. They aim to capture finegrained information with the addition of GMML as an auxiliary task. MCSSL\cite{mcssl} propose a framework which captures information at different levels. They use GMML to capture finegrained information and extend DINO\cite{dino} based clustering loss to patches to capture local semantics. iBoT\cite{ibot} proposes to extend DINO to patches but does not reconstruct masked images at pixel level. 

Different from these methods [Method name] is different from other works by introducing auxiliary pseudo labelling pretext task to a sparse encoder based MAE where the main pretext task is MIM. We also change reconstruction target from pixels to tokens. We also extend the concept of multi fold masking to clustering and propose multi fold clustering. We also differ from clustering based methods by utilising simple augmentations like cropping and horizontal flip. 



==> sec/3_methodology.tex <==
\section{Methodology}
\label{sec:methodology}
Our method is an auto-encoder model where the student encoder is a ViT \cite{vit} and the decoder consists of few transformer layers. The student decoder generates token embeddings at the output of decoder which are then passed through projection head to generate cluster assignments. The targets for reconstruction and clustering are generated by two disentangled teacher encoders where the cluster teacher generates cluster assignments from the outputs of a projection head and the token teacher acts as a code-book which generates target tokens. We use a multi fold masking strategy introduced by SdAE \cite{sdae} but introduce a multi fold class and patch level clustering which compares class clusters across multiple folds. The class level clustering enables the network to learn instance level discrimination which is absent in other MIM based methods like MAE\cite{mae}, SimMIM \cite{simmim}. Our patch level clustering learns local patch level discrimination which is different from our token level reconstruction which captures global shape information similar to SdAE \cite{sdae}. In addition our encoders generate output from multiple intermediate levels to capture finer details at lower levels and more coarser details at higher levels. We discuss the framework and the different components in detail in the following sections.

\subsection{Masked Image Modelling}

Masked Image Modelling (MIM) has emerged as a significant self-supervised learning approach in recent research \cite{sit, mae, simmim, gmml, sdae}, showcasing its effectiveness and broad utility in the domain of image processing. At its core, MIM revolves around the reconstruction of an original image from an input image that has been partially masked. In this section, we provide an in-depth discussion of our novel MIM approach, utilising vision transformers.
%Masked Image Modelling (MIM) has been explored in recent works \cite{gmml, mae, simmim, sdae} which reconstruct the original image from a masked input image. We base our student encoder, cluster teacher and token teacher on ViT \cite{vit}.  

Consider an input image $\mathbf{x} \in \mathcal{R}^{H \times W \times C}$, where $H$, $W$, and $C$ denote height, width, and the number of channels, respectively. The image is then converted into a sequence of flattened patches, resulting in a two-dimensional matrix $\mathbf{x} \in \mathcal{R}^{N \times (P^{2}.C)}$, where $N$ is the number of patches and $P\times P$ is the resolution of each patch. 
%
Subsequently, we generate a random mask $\textbf{M} ={(m_{1}, \dots, m_{N}})$ for the $N$ tokens, with each $m_{i}\in{\{0, 1\}}$, determining the tokens to be retained or discarded. 
%

For the student encoder, we input $\mathbf{\hat{x}} \in \mathcal{R}^{ (N'+1) \times (P^{2}.C)}$, where $N'$ is the number of the tokens corresponding to $m_{i}=0$ plus 1 for the class token. The output of the student encoder $\mathbf{\tilde{x}\in R}^{(N'+1) \times D}$, where $D$ is the embedding dimension of the encoder, are then passed through decoder following MAE \cite{mae} to produce decoder outputs. The objective function for reconstruction is simply a cosine similarity loss between targets and decoder output embeddings.

\begin{equation} \label{eq:recons}
    %\mathcal{L}_{m} = \frac{1}{sum(M)}\sum_{i}^{N} \frac{1}{2}( m_{i} \times (\overline{t_{rec}(\mathbf{x}_i)} - \mathbf{\tilde{x}}_i )^{2}
    \mathcal{L}_{m} = \frac{1}{N'}\sum_{i}^{N} cos\_sim( m_{i} \times (\overline{t_{rec}(\mathbf{x}_i)}, \mathbf{\tilde{x}}_i )
\end{equation}


\begin{equation} \label{eq:t_norm}
    \overline{t_{rec}(\mathbf{x}_i)} = \frac{t_{rec}(\mathbf{x}_i)-mean(t_{rec}(\mathbf{x}_i))}{\sqrt{var(t_{rec}(\mathbf{x}_i))+\epsilon}}
\end{equation}

Equation \ref{eq:recons} gives the equation for reconstruction loss where $t_{rec}$ is the teacher encoder which generates tokens. This is different from MAE which uses original input pixels as the targets. Here $\tilde{\mathbf{x}}_{i} = (\tilde{\mathbf{x}}_{1}, \dots, \tilde{\mathbf{x}}_{N})$ is the output corresponding to patches excluding the class token output $\tilde{\mathbf{x}}_{N+1}$. We use normalized teacher inputs as the targets which are given by the Equation(\ref{eq:t_norm}).

In addition we use a multi-fold masking strategy \cite{sdae} for generating targets with teacher encoder. Let $\mathbf{x^{m}}$ represent the unmasked input where $\mathbf{x}^{m}=\{\mathbf{x}_i \mid \mathbf{m}_i=0\}$. The unmasked input $\mathbf{x}^{m} \in \mathbf{R}^{(N-N') \times (P^{2}.C)}$ is split in $K$ folds ($\mathbf{x}^{1}, \dots, \mathbf{x}^{k}$) to which class tokens are prepended to generate multi-fold split outputs ($(t_{rec}(\mathbf{x}^{1}), \dots, t_{rec}(\mathbf{x}^{k})$). The output patches excluding that of class token of these multifold outputs is utilised in Equation(\ref{eq:recons}). 

\subsection{Disentangled Teachers}
Several works like \cite{sit, mcssl, ibot} explore combining their primary pretext task clustering/contrastive learning with auxiliary pretext task of MIM. Apart from their encoders not being sparse due to use of mask tokens/zeros they utilise a single teacher for both clustering/contrastive learning and their auxiliary task MIM. 
%These methods\cite{sit, mcssl} also reconstruct at a pixel level where as we follow token level reconstruction similar to \cite{beit, ibot, sdae}. 
The models used have utilised a single teacher for both their auxiliary task and the primary pretext task which are updated with exponential moving average(EMA). We propose to use two teachers namely cluster teacher $t_{cl}$ and reconstruction teacher $t_{rec}$ that disentangle the task of generating target cluster assignments from generating target token representations. The teacher for token representation benefits from having stable teacher where the teacher is updated by EMA less frequently i.e. per epoch. The teacher for target cluster assignments performs better when updated frequently i,e, per iteration. Utilising two different teachers specialised in different pretext tasks enables us to also apply two different EMA update schedules with different frequencies. Specifically the EMA for our cluster teacher is done for each iteration with a starting momentum of $0.996$ where as the EMA of the reconstruction teacher is done for each epoch with a starting momentum of $0.96$.

\subsection{Multifold Clustering}
Mulifold masking produces noticeable improvements for downstream tasks as shown in \cite{sdae}. We aim to extend multifold masking strategy for clustering as well. Given the unmasked input $\mathbf{x}^{m} \in \mathbf{R}^{(N-N') \times (P^{2}.C)}$ we split in $K$ folds ($\mathbf{x}^{1}, \dots, \mathbf{x}^{k}$) and prepend class token to each fold. The resulting folds are passed through cluster teacher $t_{cl}$ to generate multifold cluster split outputs ($(t_{cl}(\mathbf{x}^{1}), \dots, t_{cl}(\mathbf{x}^{k})$) which include class and patch cluster assignments for each fold. Noticeably we differ from other clustering based methods by utilising a single crop and no other data augmentation than random cropping and horizontal flipping.

To generate clusters from multi fold cluster input ($\mathbf{x}^{1}, \dots, \mathbf{x}^{k}$) we pass it through the teacher encoder $t_{cl}$ which generates output tokens. These tokens are then passed through the projection head, the design of which follows MCSSL\cite{mcssl}. The projection head has multiple shared MLP layers except the last layer which is different for patch and class tokens and has a final output projection dimension of $4096$ for both patch and class token layers. To generate cluster assignments from these outputs we apply sinkhorn normalization similar to SwAV\cite{swav} but we extend it to patches in addition to class token. Let $(\mathbf{p}^{1}, \dots, \mathbf{p}^{k})$ be the patch cluster assignments and $(\mathbf{c}^{1}, \dots, \mathbf{c}^{k})$ be the class cluster assignments after projection head for different folds. 

To generate student cluster assignments we first generate $\tilde{\mathbf{x}}^{m}=\{\tilde{\mathbf{x}}_i \mid \mathbf{m}_i=0\}$ from student decoder outputs which excludes the output corresponding to class token $\tilde{\mathbf{x}}_{N+1}$. Both $\tilde{\mathbf{x}}^{m}, \tilde{\mathbf{x}}_{N+1}$ are passed through the student projection head to generate predicted cluster assignments $\mathbf{\tilde{p}}, \mathbf{\tilde{c}}$ corresponding to patch and class respectively. The cluster assignments are split into K folds to generate multifold patch prediction cluster assignments $(\mathbf{\tilde{p}}^{1}, \dots, \mathbf{\tilde{p}}^{k})$

\begin{equation} \label{eq:ptch}
        \mathcal{L}_{p} = \frac{1}{N'}\sum_{i=1}^{K}\sum_{n=1}^{}\text{H}(\mathbf{p}^{i}_{n}, \mathbf{\tilde{p}}^{i}_{n})
\end{equation}

\begin{equation} \label{eq:cls}
        \mathcal{L}_{c} = \frac{1}{K}\sum_{i=1}^{K}\text{H}(\mathbf{c}^{i}, \mathbf{\tilde{c}})
\end{equation}

To calculate the patch level clustering loss we apply cross entropy loss $H$ between different teacher patch folds $\mathbf{p}^{i}$ and student patch folds $\mathbf{\tilde{p}}^{i}$ which is given by Equation(\ref{eq:ptch}). For class level clustering loss we calculate loss between the single student class cluster assignment $\mathbf{\tilde{c}}$ with each fold of teacher class cluster assignment $\mathbf{c}^{i}$. The Equation(\ref{eq:cls}) provides formulation for class clustering loss. 

\subsection{Hierarchical feature capture in encoder and loss}
To encode information at different levels of feature hierarchy we propose to combine information at different layers of the both teacher encoders and the student encoder to generate output embeddings. Let $\mathbf{\tilde{x}^{\it{l}}\in R}^{(N+1) \times D}$ be the output at layer $\it{l}$ of the student encoder. The final output is given as the summation of the set of $L$ layer outputs $\mathbf{\tilde{x}}=\sum_{l=\it{L}}(\mathbf{\tilde{x}^{\it{l}}})$. We set $L=\{4, 6, 8, 12\}$ by default and this procedure is also followed for cluster teacher and reconstruction teacher. The layers at lower level focus on finer details in addition to capturing small scale objects. The layers at higher layers capture more semantic features and also capture large scale objects. 

\begin{equation} \label{eq:loss}
        \mathcal{L} = \lambda_{m}*\mathcal{L}_{m} + \lambda_{c}*\mathcal{L}_{c} + \lambda_{p}*\mathcal{L}_{p}
\end{equation}


The final loss is given by Equation(\ref{eq:loss}) is the combination of reconstruction loss $\mathcal{L}_{m}$, class clustering loss $\mathcal{L}_{c}$ and patch clustering loss $\mathcal{L}_{p}$ with scaling factors $\lambda_{m}, \lambda_{c}, \lambda_{p}$ respectively.


%You must include your signed IEEE copyright release form when you submit your finished paper.
%We MUST have this form before your paper can be published in the proceedings.

%Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
%\url{https://www.computer.org/about/contact}.

==> sec/4_experiments.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{l | c c c c c c c}
 Method & Backbone & FLOPs (G) & Param. (M) & Supervision & Pretrain Epochs & Finetuning & Linear Evaluation\\
 \hline
 ViT\cite{vit} & ViT-B & 17.5 & 86 & RGB & - & 79.9 & -\\  
 BEiT\cite{beit} & ViT-B & 17.6 & 87 & DALL-E & 800 & 83.2 & 37.6\\
 CAE\cite{cae} & ViT-B & 17.5 & 86 & DALL-E & 800 & 83.6 & 68.6\\
 MaskFeat\cite{maskfeat} & ViT-B & 17.5 & 86 & HOG & 300 & 83.6 & -\\
 iBOT\cite{ibot} & ViT-B & 17.5 & 86 & Momentum & 1600 & 84.0 & -\\
 MCSSL\cite{mcssl} & ViT-B & 17.5 & 86 & Momentum & 800 & 84.0 & -\\
 MAE\cite{mae} & ViT-B & 17.5 & 86 & Momentum & 800 & 83.6 & 67.8\\
 SdAE\cite{sdae} & ViT-B & 17.5 & 86 & Momentum & 300 & 84.1 & 64.9\\
 Ours & ViT-B & 17.5 & 86 & Momentum & 300 & 84.0 & -\\
\end{tabular}
\caption{Temporary Table for results on Imagenet-1K.}
\end{table*}



\begin{table*}[h]
\centering
%\resizebox{0.99\linewidth}{!} {
\begin{tabular}{l  c c c c c c} 
 \hline
 Method & Backbone & Flowers & Pets & Cars & Cifar-10 & Cifar-100 \\ 
 \hline 
 Supervised & ViT-B & 98.2 & -- & 92.1 & 99.0 & 89.5 \\
MoCov3 & ViT-B & 97.7 & 92.3 & 93.0 & 98.2 & 86.6 \\ 
DINO & ViT-B & 97.8 & 89.4 & 93.1 & 99.0 & 90.5 \\
iBoT & ViT-B & 98.6 & 93.1 & \textbf{94.0} & 99.1 & 90.7\\
Ours & ViT-B  &  & &  &  &  \\ 
 \hline
\end{tabular}
%}
\caption{Transfer learning by finetuning pretrained models with the ViT-B/16 backbone on diverse datasets. We report top-1 accuracy.}
\label{table:small_finetune}
\end{table*}

\section{Experiments}
\label{sec:experiments}
We base our experiment setup on pretraining first and finetuning next to evaluate our approach across several downstream tasks and datasets. We pretrain our model based on Imagenet-1K\cite{imagenet} following previous works\cite{dino, ibot, mae}. We evaluate our model on multiple downstream tasks like multi class classification, semantic segmentation, objection detection, instance segmentation. The pretraining for Imagenet-1K is done for 800 epochs with AdamW\cite{adamw} as the optimiser. The default image size is set to $224\times 224$ and the patch size for ViT\cite{vit} is set to $16$. The masking ratio is set to $75\%$ following MAE, the learning rate is set to $2.666e-4$ and warmup epochs to $60$. The staring, ending momentum for momentum schedule of reconstruction teacher is set to $0.96, 0.99$ respectively where the momentum update is done for each epoch. The staring, ending momentum for momentum schedule of cluster teacher is set to $0.996, 1$ respectively where the momentum update is done for each iteration. 





\subsection{Results on multi class classification}
We evaluate our model on Imagenet-1K\cite{imagenet} by finetuning for $100$ epochs on ViT-B. We set a base learning rate of $5e-4$  warmup epochs to $5$.  We utilise an effective batch size of $1024$ with weight decay set to $0.05$ and layer decay to $0.65$. We compare our model to other SSL methods like DINO\cite{dino}, BEiT\cite{beit}, MAE\cite{mae} on finetuning. 


We also evaluate on other smaller datasets like Pets, Cars, Cifar10, Cifar100. The finetuning is done for $1000$ epochs with a similar settings to DINO\cite{dino}. When compared against other methods we find that our method performs better. 


\subsection{Results on semantic segmentation}
We perform the finetuning and evaluation for semantic segmentation on ADE20K dataset. We follow previous SSL approaches\cite{dino, moco, simclr} by utlising Upernet\cite{upernet} as the task layer. We follow MAE\cite{mae} for setting the schedule and learning rate. Semantic segmentation shows the capability of the network to capture semantic details at various levels and provides for a good dowsntream task. 


\begin{table*}[h]
\centering
%\resizebox{0.99\linewidth}{!} {
\begin{tabular}{l  c c c c c} 
 \hline
 Method & Backbone & Pretrain Epochs & FLOPs (G) & Params (M) & mIoU \\ 
 \hline 
 Supervised & ViT-B & 300 & 606 & 164 & 47.0\\
MoCov3 & ViT-B & 300 & 606 & 164 & 47.2\\
DINO & ViT-B & 400 & 606 & 164 & 47.2\\
BEiT & ViT-B & 300 & 606 & 164 & 45.5\\
BEiT & ViT-B & 800 & 606 & 164 & 46.5\\
MAE & ViT-B & 300 & 606 & 164 & 45.8\\
MAE & ViT-B & 1600 & 606 & 164 & 48.1\\
%iBoT & ViT-B & 1600 & 606 & 164 & 50.0\\
CAE & ViT-B & 300 & 606 & 164 & 47.7\\
SdAE & ViT-B & 300 & 606 & 164 & 48.6\\
Ours & ViT-B  &  & &  &   \\ 
 \hline
\end{tabular}
%}
\caption{Transfer learning by finetuning pretrained models with the ViT-B/16 backbone on diverse datasets. We report top-1 accuracy.}
\label{table:sem_seg}
\end{table*}



\begin{table*}[h]
\centering
%\resizebox{0.99\linewidth}{!} {
\begin{tabular}{l  c c c c c c c c} 
 \hline
 \multirow{2}{*}{Method} &  \multirow{2}{*}{Backbone} & \multirow{2}{*}{Pretrain Epochs} & \multicolumn{3}{c|}{Object detection} & \multicolumn{3}{c}{Instance Segmentation}\\ %\cline{4-11}
  &  &  & $AP^{b}$ & $AP^{b}_{50}$ & $AP^{b}_{70}$  & $AP^{m}$ & $AP^{m}_{50}$ & $AP^{m}_{70}$\\ 
 \hline 
 Supervised & ViT-B & 300 & 46.9 & 68.9 & 51.0 & 41.5 & 65.5 & 44.4\\
MoCov3 & ViT-B & 300 & 45.5 & 67.1 & 49.4 & 40.5 & 63.7 & 43.4\\
DINO & ViT-B & 400 & 46.8 & 68.6 & 50.9 & 41.5 & 65.3 & 44.5\\
BEiT & ViT-B & 300 & 39.5 & 60.6 & 43.0 & 35.9 & 57.7 & 38.5\\
BEiT & ViT-B & 800 & 42.1 & 63.3 & 46.0 & 37.8 & 60.1 & 40.6\\
MAE & ViT-B & 300 & 45.4 & 66.4 & 49.6 & 40.6 & 63.4 & 43.7\\
MAE & ViT-B & 1600 & 48.4 & 69.4 & 53.1 & 42.6 & 66.1 & 45.9\\
%iBoT & ViT-B & 1600 & 51.2 & -- & -- & 44.2 & -- & --\\
CAE & ViT-B & 300 & 48.0 & 68.7 & 52.7 & 42.3 & 65.6 & 45.4\\
SdAE & ViT-B & 300 & 48.9 & 69.6 & 53.3 & 43.0 & 66.2 & 46.2\\
Ours & ViT-B  &  & &  &   \\ 
 \hline
\end{tabular}
%}
\caption{Transfer learning by finetuning pretrained models with the ViT-B/16 backbone on diverse datasets. We report top-1 accuracy.}
\label{table:sem_seg}
\end{table*}


\subsection{Results on object detection, instance segmentation}
Following MAE\cite{mae} we finetune our architecture on COCO dataset\cite{mscoco}. We use Mask R-CNN\cite{maskrcnn} and we also apply FPN\cite{fpn} to train the network. The learning rate and the schedule used follows MAE\cite{mae}. 

==> sec/5_ablation.tex <==
\section{Ablation}
\label{sec:ablation}
We conduct ablation study on Imagenet-1K with ViT-S as the backbone. We study the usage of multiple teachers for different pretext task. We explore the effect of EMA having different update frequencies i.e. per epoch or per iteration on each of the teacher. We also explore the effect of longer pretraining and different losses in our architecture. Augmentations are generally used in all clustering frameworks\cite{dino, mcssl, sit}. We explore the effect of different augmentations on the model as we have an auxiliary pretext task of clustering. 


\begin{table}[h]
\centering
\small
\begin{tabular}{c | c c}
 Method & Backbone & In-1\%\\
 \hline
 SdAE & ViT-S & 51.75\\
Single Techer(Per iteration) & ViT-S & 51.91\\  
Single Techer(Per epoch) & ViT-S & 51.04\\
 Recons Teacher + Cluster Teacher (default) & ViT-S & 52.85\\
\end{tabular}
\caption{Temporary results of our method compared to a single teacher which generates both cluster assignments and target tokens. The single teacher is updated is either per epoch or per iteration and we also compare against the original SdAE.}
\end{table}


\begin{table}[h]
\centering
\small
\begin{tabular}{c | c c c}
 Backbone & Initial Momentum & Final Momentum & In-1perc\\
 \hline
 ViT-S & 0.96 & 1 &  51.81\\  
 ViT-S & 0.996 & 1 & 52.85\\
\end{tabular}
\caption{Temporary results of using different momentums for our cluster teacher. Large momentums work better for generating cluster assignments.}
\end{table}


\begin{table}[h]
\centering
\small
\begin{tabular}{c | c c}
 Method & Backbone & In-1perc\\
 \hline
 cls+periter & ViT-S & 51.91\\  
 nocls+periter & ViT-S & 51.64\\
\end{tabular}
\caption{Temporary results of no class token vs class token cluster loss}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{c | c c}
 Method & Backbone & In-1K\\
 \hline
 SdAE & ViT-B & 82.19\\  
 Cluster on patches & ViT-B & 81.93\\
\end{tabular}
\caption{Temporary results of only cluster loss}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{c | c c}
 Method & Backbone & In-1K\\
 \hline
 MAE & ViT-B & 80.28\\  
 MAE+int & ViT-B & 80.45\\
\end{tabular}
\caption{Effect of intermediate connections on Imagenet-1K.}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{c | c c}
 Method & Backbone & In-1perc\\
 \hline
 CenterCrop+HFlip & ViT-S & 52.85\\  
 +Guassian+Grayscale & ViT-S & 51.24\\
 +Solarization& ViT-S & 50.89\\
\end{tabular}
\caption{Effect of different augmentations with our framework}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{c | c c}
 Method & Backbone & In-1perc\\
 \hline  
 Multifold & ViT-S & 52.85\\
 No Multifold& ViT-S & \\
\end{tabular}
\caption{Effect of different multifold clustering vs normal clustering}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{c | c c c}
 Backbone & Epoch & In-1perc\\
 \hline  
ViT-S & 100 epochs& \\
ViT-S & 300 epochs& \\
ViT-S & 800 epochs& \\ 
\end{tabular}
\caption{Effect of longer pretraining}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{c | c c c c}
 Method & Backbone & Pretraining Time & Throughput & \\
 \hline  
iBoT\cite{ibot} & ViT-B & & \\
MAE\cite{mae} & ViT-B & & \\
Ours(Single Teacher) & ViT-B & & \\
Ours(Disentangled Teachers) & ViT-B & & \\
\end{tabular}
\caption{Throughput\& pretrain time comparison of different methods with ours. Our method with only a single teacher generates both target clusters and tokens. The throughput calculations are done on $8$ V-100s under similar settings.}
\end{table}

\noindent
\textbf{Effect of Multiple Teachers and EMA update frequency}
Clustering and token reconstruction can be performed with a single teacher. We study the effects of having a single teacher with both reconstruction and clustering. The update frequency of this teacher can be done for an epoch or an iteration. We compare this teacher with each update done for each iteration against the model where it is done for each epoch. When compared with our disentangled teacher strategy where the cluster teacher generates cluster assignments and the reconstruction teacher generates token level representation, our strategy performs the best. Our cluster teacher is updated frequently per each iteration and the reconstruction teacher is updated per each epoch. We find that reconstruction teacher performs best when updated per epoch and cluster teacher performs better when update per each iteration. Having two teachers enables us to decouple the EMA schedules for different pretext tasks and provide a more stable training. Table\ref{} provides the results for the above ablation experiments.

\noindent
\textbf{Effect of Different schedules on clustering teacher}
We study the effect of different momentum schedules for cluster teacher. We consider a schedule with initial momentum of $0.96$ and final momentum of $1$ and different schedule with a initial momentum of $0.996$ and similar final momentum of $1$. The schedule with a momentum of $0.996$ performs better and shows that the cluster teacher requires not only frequent updates but larger ones. This further shows the requirement of a disentangled teachers as different pretext task require different teachers with different properties.


\noindent
\textbf{Effect of different clustering loss terms}
We study the effects of different auxiliary pretext clustering loss terms on the performance of the model. We find that when we apply only class clustering loss on patches with i.e. $\lambda_{p}=0$, we get a lower accuracy. We find that when we apply both class and patch level clustering it leads to a slight improvement in performance.

\noindent
\textbf{Effect of Multifold clustering}
We also study the effects of applying multifold clustering and compare it to normal clustering. Multifold masking\cite{sdae} shows that keeping the sufficient mutual information provides for a better encoder. We introduce similar concept to clustering and study its effects. We find that following multifold clustering generates better results than without application of multifold clustering.


\noindent
\textbf{Effect of hierarchical feature capture}
Our encoder is designed to generate output embeddings by considering the outputs at various layers in a ViT\cite{vit} model. Specifically we combine the features from layers $[4, 6, 8, 12]$ and add them to generate the output embeddings. The lower layers generally contain lower level information and higher layers contain semantic information. Lower layer also tend to capture smaller objects and the higher layers focus on large scale objects. By capturing information at multiple levels we are able to develop a better model which captures hierarchical information. To prove this, we train MAE\cite{mae} with ViT-B\cite{vit} as the encoder and compare it with MAE which has hierarchical skip connections at layers $[4, 6, 8, 12]$. When trained with pretraining epochs of $100$ and finetuned for $50$ epochs the MAE with hierarchical connections works best. 

\noindent
\textbf{Effect of different augmentations}
Generally  MAE does not use any harsh augmentations except for center crop and horizontal flip. Augmentations like guassian blur, solarization and grayscale are regularly used in frameworks which use clustering\cite{dino, sit, mcssl, ibot}. We apply different augmentations to our framework and pretrain the model for $100$ epochs and finetune it for $50$ epochs to compare the effect of augmentation. Even with auxiliary pretext clustering task our frameworks prefers simple augmentations like center crop and horizontal flip.

\noindent
\textbf{Effect of longer pretraining}
We find that clustering based methods are trained for $800$ epochs with multiple views while MAE\cite{mae} is trained for $1600$ epochs. SdAE, CAE which are based on mae are trained for $300$ epochs and saturate after that period. We find that our model when trained for longer produces better downstream performance. We pretrain ViT-S for 100, 300, 800 epochs respectively and find that longer training works well for our model,


==> sec/6_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We propose an MIM model with a auxiliary pretext task of psuedo label generation. The auxiliary task imbues the network with instance discrimination at global and local level. We find that naive addition of auxiliary pretext task does not directly produce any additional gains due to the differing nature of teachers required for pseduo labelling with clustering and token based reconstruction. We propse to adopt two disentangled teacher namely cluster teacher to generate cluster assignments and token reconstruction teacher to generate target tokens. We find that token reconstruction requires more stable teacher, hence we perform EMA update for the token teacher at each epoch. In contrast, the cluster teacher requires more frequent EMA updates where the update is done at each iteration. We also emphasise the need to capture information at multiple levels to generate a better encoder. In future we aim to extend this work to multimodality and the study the behivour of teachers for different multimodal tasks. 
